Fortunately, Discourse Markers Can Enhance Language Models for Sentiment Analysis

In recent years, pretrained language models have revolutionized the NLP world, while achieving state of the art performance in various downstream tasks. However, in many cases, these models do not perform well when labeled data is scarce and the model is expected to perform in the zero or few shot setting. Recently, several works have shown that continual pretraining or performing a second phase of pretraining (inter-training) which is better aligned with the downstream task, can lead to improved results, especially in the scarce data setting. Here, we propose to leverage sentiment-carrying discourse markers to generate large-scale weakly-labeled data, which in turn can be used to adapt language models for sentiment analysis. Extensive experimental results show the value of our approach on various benchmark datasets, including the finance domain. Code, models and data are available at https://github.com/ibm/tslm-discourse-markers.

==> OLD_Experimental_Setup.tex <==
\section{Experimental Setup}

\subsection{The Unlabeled Corpora}
\label{sec:corpora}

\paragraph{The General Corpus (\gencorpus{})} 
Our proposed solution relies on a large corpus of unlabeled text. We use a corpus of some $400$ million newspaper and journal articles\footnote{From the LexisNexis 2011-2018 corpus,https://www.lexisnexis.com/en-us/home.page} breaking the articles into sentences, and indexing these sentences.
We focus on English sentences\footnote{have a high probability of being English ($> 75\%$) using Fast-Text langid from \cite{grave-etal-2018-learning}} and following \cite{sileo-etal-2019-mining} we use only sentences which are $3-32$ tokens in length and have balanced parentheses.

\paragraph{The \fincorpus{}} 
From the General Corpus we can also define a sub-corpus that is focused on the financial domain, using a provided metadata topic field, and filtering only for articles from the topic 'finance'.
%In some places in this work we are also interested to train using a general model which excludes the financial domain, in order to test how we can adapt to a new domain that is not included in the data used for training the general sentiment models. We define \nonfincorpus{} simply as \gencorpus{} minus \fincorpus{}.

\paragraph{The \sportscorpus{}} 
Similarly to the above description for the \fincorpus{} but filtering for articles from the topic 'sports'.

\paragraph{The \scicorpus{}} Since we are interested in scientific articles from scientific journals only, we define this domain as any article in \gencorpus{} that was published in one of the journals included in the list of journal impact factors\footnote{ https://www.scimagojr.com/journalrank.php}. 
%Analogously to the financial domain we define \nonscicorpus{} simply as \gencorpus{} minus \scicorpus{}.

\subsection{Inter-training Details}
The inter-training step (figure \ref{fig:sketch}) consists of fine tuning BERT using weakly labeled data.
For inter-training \genmodel{}, we obtain a total of $1876614$ weakly labeled sentences, by using the list of sentiment-related DMs, $L_g$, over sentences in the general corpus, $C_g$, as described in section \ref{section:the_alg}. 
For the number of weakly labeled samples used for training domain-specific sentiment models, see table \ref{sup-tab:sizes}. In all cases we divide the samples into training ($80\%$), development ($10\%$) and test ($10\%$) sets. 
We perform the inter-training with a batch size of 32. To determine the number of training epochs we use early stopping, and train until the improvement of accuracy on the development set is lower than 1e-3. 
We employ an Adam optimizer with a learning rate of 5e-5, $\beta_1$ of 0.9, $\beta_2$ of 0.999, and $\epsilon$ of 1e-06. Training is performed on two V100 GPUs. 


\subsection{Evaluation Details}
\label{sec:eval}

To evaluate the sentiment language models, we test the zero and few shot settings on the below datasets.
For zero shot we use the classification layer obtained from inter-training. 
For the few shot finetuning we sample from 16 to 1024 examples from the training dataset. 
To support training on small datasets, we train with batch size of 16. We repeat each experiment five times with different random seeds, each time selecting different examples for fine tuning. We use an Adam optimizer as described above for the inter-training.

\subsubsection{Datasets}

The datasets used for evaluation are presented in table \ref{tab:datasets}. All datasets contain sentences that are labeled for sentiment, either positive or negative. \amazonds, \sstds and \yelpds consist of review sentences. \fbpds{} is comprised of sentence from a financial domain. %, and \citationds contains sentences from ACL papers. 
Most of these datasets provide more than two possible labels, so we adjust the datasets for the binary sentiment classification task. 
%For \citationds and \fbpds contain sentences that are labeled as neutral, thus we remove them from our training and evaluation sets. \yelpds and \amazonds contain five different labels that are infect the sentiment ratings of each sentence. We leave only sentences with the lowest and highest scores, considering those as negative and positive labels.  
%Specifically, \citationds{} and \fbpds{} contain sentences that are labeled as neutral, which we remove from the training and test sets. 
Specifically, \fbpds{} contains sentences that are labeled as neutral, which we remove from the training and test sets. 
 \amazonds{}  and \yelpds{} contain five different labels that are the sentiment ratings of each sentence ("stars"). We leave only sentences with the lowest and highest scores, considering those as negative and positive labels.
For fine tuning models we use up to $1024$ examples from the training set, except in \citationds{} which contains less examples. For testing we use the entire test set.


\begin{table}[h!]
\begin{center}
\begin{tabular}{l| l |l} 
 \hline
 \textbf{Dataset} & 
 \textbf{Domain} &
  \textbf{Test set size} \\ 
 \hline
 \amazonds{} & Product reviews & 2K \\ 
 \hline
\yelpds{}  & Business reviews &  20K \\ 
\hline
\sstds{} & Movie reviews &  1821 \\ 
\hline
\fbpds{}  & Financial documents &  691\\
\hline
%\citationds{}  & Scientific publications & 217\\
%\hline
\end{tabular}
\end{center}
%\caption{Datasets used for evaluation. References for the datasets are as follows, by the order appearing in the table: \cite{marc_reviews}, \cite{wang-etal-2018-glue}, \cite{yelp_dataset}, \cite{Malo2014GoodDO}, \cite{athar:2011:SS}.
\caption{Datasets used for evaluation. References for the datasets are as follows, by the order appearing in the table: \cite{marc_reviews}, \cite{yelp_dataset}, \cite{wang-etal-2018-glue}, \cite{Malo2014GoodDO}.
\label{tab:datasets}
}
\end{table}

\subsubsection{Baselines}
\label{sec:baselines}
\ranit{SAY A FEW WORDS ABOUT FINBERT}
\sentix{}\cite{lek2012sentix} is a sentiment-aware pre-trained language model that is aimed to perform cross domain sentiment analysis. 
Unlike many language models, including our model and BERT, \sentix{} leverages a supervision signal that is not part of the text itself, namely the human ratings ("stars") given in Amazon and Yelp. 
In that sense, it is not a true baseline for our model since we are interested in proposing a method that does not rely on any human annotation per sample, even it is "free". Rather, the method can be generalised to any domain, relying only on the text itself, and not on lebels that are available only in a specific domain.
Nevertheless, we present results of fine-tuning \sentix{} on the datasets we used for evaluation excluding \amazonds{} and \yelpds{}, as these were part of its training set, and it is not possible to determine whether the test set instances were excluded from its training. \ranit{verify and rethink if we really want to say it is not a baseline}


%zero shot we use the classification layer obtained from inter-training.
%finetuning:
%5 repeats seed first=123 each run add 1.
%, sampled  from training set of the dataset
%10 epochs
%train batch size =16 (edited) 




%finetuning:
%5 repeats
%sample sizes 0-1024 - mention that taken from training set of the dataset (we do not give the training set size but maybe mention that all training sets are >1024)
%10 epochs
%we use the default bert parameter values, lr, scheduler...





%\textbf{\citationds} \cite{athar:2011:SS} consists sentences extracted from ACL papers. We consider only polar sentence (labeled as positive or negative),and ignore all the neutral sentence. We split the corpus into train and test set, with 6989 and 1747 instances, respectively.

%\textbf{\fbpds} \cite{Malo2014GoodDO} consist of sentence extracted from a financial domain labeled for sentiment. The dataset consist of several views, with a different inter annotators agreement for each view. For this work, we use the view with an agreement of at least 75\%. Similarily to \citationds, we remove sentences that are labeled as neutral. We split the corpus into train and test set, with 2762 and 691 instances, respectively.  

%\textbf{\yelpds} \cite{yelp_dataset} consists of Yelp reviews scored between 0 to 4. We only use reviews that are scored with 0 or 4 (that is, the most polar scores) with the standard train and test split provided for this dataset with 260K and 20K instances, respectively.


%\textbf{\amazonds} \cite{marc_reviews} consist of the English part of Amazon reviews corpus. As for \yelpds we maintain only the most polar labels (one and five starts), resulting in a training set of size 80, and dev and test sets, each of 2K examples.

%\textbf{\sstds} \cite{wang-etal-2018-glue} consists of sentences from movie reviews, along with an annotation of their sentiment (positive and negative). The dataset is split into a training set of size 67349, a validation set of size 872 and a test set of size 1821.


==> OLD_Results.tex <==
\section{Results}
We now evaluate the performance of our general sentiment model, \genmodel{}, which we release to the community, as well as the performance of the model adapted to the finance domain.
Since our main focus is on the zero and few-shot setting, we report fine-tuning results for $0$ up to $1024$ training examples in all cases studied below.

\subsection{\genmodel{}}
\label{sec:resgenmodel}


\begin{comment}
\begingroup
\setlength{\tabcolsep}{1pt} % Default value: 6pt
\renewcommand{\arraystretch}{0.2} % Default value: 1

\begin{figure*}
\begin{tabular}{ccccc}
    \begin{tabular}{c}
    % \\ base \\ tiny
    \\   \raisebox{17ex}{base} \\ \raisebox{-1.5ex }{tiny}
 \end{tabular} &
 
 \begin{tabular}{c}
    \amazonds \\ \includegraphics[width = 1.6in]{Figures/fig2/amazon_en15_base.png} \\
    \includegraphics[width = 1.6in]{Figures/fig2/amazon_en15_tiny.png}
 \end{tabular} &
 
  \begin{tabular}{c}
    \yelpds  \\ \includegraphics[width = 1.6in]{Figures/fig2/yelp04_base.png} \\
    \includegraphics[width = 1.6in]{Figures/fig2/yelp04_tiny.png}
 \end{tabular} &
 
  \begin{tabular}{c}
    \sstds  \\ \includegraphics[width = 1.6in]{Figures/fig2/sst2_base.png} \\
    \includegraphics[width = 1.6in]{Figures/fig2/sst2_tiny.png}
 \end{tabular} &


  \begin{tabular}{c}
    \fbpds  \\ \includegraphics[width = 1.6in]{Figures/fig2/fpb75_base.png} \\
    \includegraphics[width = 1.6in]{Figures/fig2/fpb75_tiny.png}
    \end{tabular} 

\end{tabular}
%\caption{Performance of \genmodel{} and baselines on five datasets given different amounts of training examples. Left column: base-size models. Right column: tiny-size models.}
\caption{Performance of \genmodel{} and baselines on four datasets given different amounts of training examples. Top row: base-size models. Bottom row: tiny-size models. Shaded area indicates the standard deviation over the five seeds (see section \ref{sec:eval} for details). Dashed horizontal lines indicate the prior of the common class in the dataset.}
\label{fig-general}
\end{figure*}
\endgroup
\end{comment}


\begingroup
\setlength{\tabcolsep}{1pt} % Default value: 6pt
\renewcommand{\arraystretch}{0.2} % Default value: 1

\begin{figure*}
\begin{tabular}{ccc}
    \begin{tabular}{c}
    % \\ base \\ tiny
    \\   \raisebox{28ex}{ \amazonds} \\ \raisebox{28ex }{\yelpds}
    \\  \raisebox{1ex }\sstds \\   \raisebox{-29ex }\fbpds
 \end{tabular} &
 
 \begin{tabular}{c}
    base \\ \includegraphics[width = 2.5in]{Figures/fig2/amazon_en15_base.png} \\
    \includegraphics[width = 2.5in]{Figures/fig2/yelp04_base.png}
    \\ \includegraphics[width = 2.5in]{Figures/fig2/sst2_base.png} \\
    \includegraphics[width = 2.5in]{Figures/fig2/fpb75_base.png}
 \end{tabular} &
  \begin{tabular}{c}
    tiny  \\ \includegraphics[width = 2.5in]{Figures/fig2/amazon_en15_tiny.png} \\
    \includegraphics[width = 2.5in]{Figures/fig2/yelp04_tiny.png}
   \\ \includegraphics[width = 2.5in]{Figures/fig2/sst2_tiny.png} \\
    \includegraphics[width = 2.5in]{Figures/fig2/fpb75_tiny.png}
    \end{tabular} 
\end{tabular}
%\caption{Performance of \genmodel{} and baselines on five datasets given different amounts of training examples. Left column: base-size models. Right column: tiny-size models.}
\caption{Performance of \genmodel{} and baselines on four datasets given different amounts of training examples. Left column: base-size models. Right column: tiny-size models. Shaded area indicates the standard deviation over the five seeds (see section \ref{sec:eval} for details). Dashed horizontal lines indicate the prior of the common class in the dataset. \finbert{} and \sentix{} are available only in the base size.}
\label{fig-general}
\end{figure*}
\endgroup




We first test the performance of both the base and tiny versions of the general sentiment model (\genmodelbase{} and \genmodeltiny{}) on datasets from multiple domains. 
Figure \ref{fig-general} shows the accuracy of the \genmodelbase{} (left column) and \genmodeltiny{} (right column), for all datasets, vs. the number of examples used for fine tuning. 
The accuracy is compared to that of the vanilla BERT -- base and tiny respectively. 
%For the \fbpds{} and \citationds{} datasets, we add the corresponding domain specific versions of \bertbase{} -- \finbert{} and \scibert{}, respectively. 
For the \fbpds{} dataset, we add the corresponding domain specific version of \bertbase{} -- \finbert{}\cite{Araci2019FinBERTFS}. 
Where applicable, we also add the results of the \sentix{} model, although it is not fully comparable to the other models -- see discussion below.


In all datasets %except \citationds{}, 
\genmodel{} significantly outperforms the BERT baselines, including the finance-specific \finbert{}, especially when the number of examples used for fine tuning is very small.
The gain in performance is even more significant when focusing on the tiny architecture. 
This is especially evident in the \fbpds{} dataset, where \berttiny{} completely fails to learn with up to 256 examples, whereas the \genmodeltiny{} is able to learn with as few as 16 examples. A similar trend can be seen for the \sstds{} dataset.

While \sentix{} significantly outperforms BERT, and to some extent our model in the review dataset \sstds{}, it loses its advantage when tested on the finance domain. This supports the notion that our approach, which relies only on the meaning of words in the language, was able to produce a more general model than \sentix{}, which relied on using domain-specific, and external-to-text signals.
%showing that indeed, training using the domain-specific labels ("stars" in reviews), fails to generalize.
Furthermore, even on the \sstds{} dataset, it suffers from very unstable results in the lower range of the number of examples -- compare the shaded area of \sentix{} to our \genmodel{}.
\ranit{need to go over the sentix discussion}

Thus, overall, our DM-based sentiment model, dramatically improves sentiment classification performance for both small and large language models. 
It is striking to note that the advantage of our approach is such, that even the tiny version of \genmodel{} outperforms 
the much larger \bertbase{} baseline.





% \begingroup
% \setlength{\tabcolsep}{1pt} % Default value: 6pt
% \renewcommand{\arraystretch}{0.2} % Default value: 1

% \begin{figure}
% \begin{tabular}{ccc}
% & Base & Tiny \\
% \rotatebox[origin=lt]{90}{\amazonds}&
% \includegraphics[width = 1.6in]{Figures/plots/amazon_en15_base.png}&
% \includegraphics[width = 1.6in]{Figures/plots/amazon_en15_tiny.png} \\ 
% \rotatebox[origin=lt]{90}{\yelpds} &
% \includegraphics[width = 1.6in]{Figures/plots/yelp04_base.png} &
% \includegraphics[width = 1.6in]{Figures/plots/yelp04_tiny.png} \\
% \rotatebox[origin=lt]{90}{\sstds } &
% \includegraphics[width = 1.6in]{Figures/plots/sst2_base.png} &
% \includegraphics[width = 1.6in]{Figures/plots/sst2_tiny.png} \\
% \rotatebox[origin=lt]{90}{\fbpds} &
% \includegraphics[width = 1.6in]{Figures/plots/fpb75_base.png} &
% \includegraphics[width = 1.6in]{Figures/plots/fpb75_tiny.png}\\
% %\rotatebox[origin=lt]{90}{\citationds}&
% %\subfloat{\includegraphics[width = 1.5in]{Figures/plots/citation_2cls_base.png}} &
% %\subfloat{\includegraphics[width = 1.5in]{Figures/plots/citation_2cls_tiny.png}} %\\

% \end{tabular}
% %\caption{Performance of \genmodel{} and baselines on five datasets given different amounts of training examples. Left column: base-size models. Right column: tiny-size models.}
% \caption{Performance of \genmodel{} and baselines on four datasets given different amounts of training examples. Left column: base-size models. Right column: tiny-size models. Shaded area indicates the standard deviation over the five seeds (see section \ref{sec:eval} for details). Dashed horizontal lines indicate the prior of the common class in the dataset.}
% \label{fig-general-old}
% \end{figure}
% \endgroup

%\subsubsection{Comparison to the \sentix{} Model}





%\subsection{Adaptation to a New Domain}
\subsection{Finance-Specific Sentiment Models}

In section \ref{sec:resgenmodel} we saw that \genmodel{} improves results over baselines on all datasets, including the finance dataset, \fbpds{}.
Here we investigate whether adapting \genmodel{} to a new domain, can further improve accuracy over the general model.
We choose to study this on the financial domain since.... \ranit{finish this part}
As we are interested in studying the scenario of adapting to a new domain, which is possibly not covered by the data used to train \genmodel{}, and since the corpus used to train \genmodel{} does contain some financial documents, we generate a variant of the general model excluding the finance domain. 
This model, denoted by \genmodelnonfin{}, is trained analogously to \genmodel{}, except we exclude financial documents from \gencorpus{} before using it. We denote this simulated model by \genmodelnonfin{}. Naturally, we do not expect a user to train such a model, it is used here only to ensure the results we obtain may be generalized to domains not in the general corpus.

Leveraging \genmodelnonfin{} and $L_{fin}$, we generate the five versions of domain specific sentiment models described in \ref{sec:dssentmodels} (see table \ref{tab:domaindms} for the DMs in $L_{fin}$\footnote{We also use \genmodelnonfin{} instead of \genmodel{} to identify $L_{fin}$ for the reasons described above}.).
Figure \ref{fig:finzeroshot} depicts the accuracy of the finance specific sentiment models, on the finance dataset \fbpds{}, for the zero shot setting, in comparison to the accuracy of the general model, \genmodelnonfin{}.
As can be seen, indeed using the domain specific DMs rather than the general list, $L_g$, improves the accuracy, and this can be further improved by one step self-training -- see \dmodelLdP{} (where here $d=fin$).
For the few shot scenario we do not find significant differences between the models -- see \ref{fig:finresultsfull} in the appendix.



\begin{figure}
%\includegraphics[width=0.8\linewidth]{Figures/solution_sketch_new.jpg}
%\includegraphics[width=0.8\linewidth]{Figures/solution_sketch_new.jpg}
\includegraphics[scale=0.5]{Figures/zero_shots.png}
%\centering\includegraphics[scale=0.6]{Figures/sketch_table.png}
\label{fig:finzeroshot}
\caption{Performance of the general model and the various domain specific models on the finance dataset, \fbpds{}, for the zero shot setting. $\ast$: \genmodelnonfin{} is the general model when trained on a corpus not containing financial documents -- see main text for details. All models are base size. In all models the domain $d$ is finance. The dashed horizontal line indicates the prior of the common class in \fbpds{}.}
\end{figure}
\ranit{should we denote in the bar graph and the appendix graph the model names with fin everywhere instead of d??}
\ranit{in terms of notation i did not write base specifically  and only added in caption. all over we have some confusion. when we say simply sendm do we mean sendm-base or both?}


\subsubsection{Analysis of Domain Specific Sentiment DMs}
As we saw above, leveraging the finance specific DMs, was useful for adapting the sentiment model to the finance domain. 
We were interested to see how sentiment DMs in various domains differ, and have carved out several domain corpora out of the general corpus (see section \ref{sec:corpora} for details).
Table \ref{tab:domaindms} lists the sentiment-related DMs extracted from general English, $L_g$, as well as those extracted for the financial, sports and scientific domains -- $L_{fin}$, $L_{sports}$ and $L_{sci}$ respectively -- as described in section \ref{sec:domainDMs}. 
\ranit{think about how to explain that for finance and scientific we do this using the simulated sendm rather than the full one while for finance we do it over the full sendm - i think we can ignore and see my footnote above re this}
The first observation is that, although some DMs are ubiquitous across domains (e.g. 'fortunately'), many are domain-specific. For example, 'ORG CEO' ('Walmart's CEO', 'BOA's CEO', etc.), appear in $L_{fin}$ only. As may be expected, in financial documents, sentences opening with such a DM, often carry a positive sentiment, while in other domains, this DM is rather rare, and may carry no signal re sentiment. 
Interestingly, in scientific journals, the DMs 'but', 'yet' and 'however', while not specifically related to the scientific jargon, do tend to open sentences with a negative sentiment, something that does not occur in other domains. 

%\begin{table}[ht]
\begin{table*}%[ht]
  \centering
%\resizebox{0.45\textwidth}{!}{%
%\begin{tabular}{p{1cm}| p{3cm} | p{3cm} } 
\begin{tabular}{p{1.1cm}| p{7.5cm} | p{7.5cm} } 
 \hline
 \textbf{Domain}
 &  \textbf{Associated with Positive sentiment} &  \textbf{Associated with Negative Sentiment} \\ 
 \hline
 General %(Multi-domain) 
 & 'luckily', 'hopefully', 'fortunately', 'ideally', 'happily', 'thankfully'  & 'sadly', 'inevitably', 'unfortunately', 'admittedly', 'curiously' \\ 
 \hline\hline
 Finance & 'at the event', 'ORG CEO', 'under his leadership', 'luckily', 'in other business', 'fortunately', 'thankfully', 'hopefully', 'with ORG', 'in future', 'starting DATE', 'as ORG', 'once completed', 'the program', 'to achieve this', 'this way', 'ideally' & 'the problem is', 'according to police', 'unfortunately', 'the problem', 'sadly', 'worse' \\
 \hline
Sports & 'fortunately', 'luckily', 'thankfully' & 'admittedly', 'alas', 'at ordinal glance', 'inevitably', 'sadly', 'the problem', 'the problem is', 'true', 'worse' \\ 
 \hline
 Science & 'ideally', 'fortunately' & 'unfortunately', 'otherwise', 'but', 'yet', 'however' \\ 
 \hline
\end{tabular}
%}
\caption{Sentiment-related DMs. The lists below the double line are domain specific.
\label{tab:domaindms}
}
\end{table*}


%To ensure the results we show here are not affected by \genmodel{} being trained on a corpus also containing financial documents, we simulate 
%In order to study the scenario of adapting to a new domain possibly not covered by the data used to train \genmodel{}, and ensure the results we show here are not affected by \genmodel{} being trained on a corpus also containing financial documents, 





==> OLD_Sentiment_Models.tex <==
\section{DM-based Sentiment Models}
\label{section:the_alg}

\subsection{Training DM-based Sentiment Models}

\begin{figure*}
%\includegraphics[width=0.8\linewidth]{Figures/solution_sketch_new.jpg}
%\includegraphics[width=0.8\linewidth]{Figures/solution_sketch_new.jpg}
\centering\includegraphics[scale=0.3]{Figures/solution_sketch_new.png}
%\centering\includegraphics[scale=0.6]{Figures/sketch_table.png}

\caption{Overview of how DM-based sentiment models are trained.}
\label{fig:sketch}
\end{figure*}

The DM-based sentiment model relies on a large weakly labeled sentiment data set, which is automatically generated by leveraging strong associations between discourse markers and sentiment classes, as described in figure \ref{fig:sketch}.
Given a corpus $C$ and a list $L$, of DMs that signal either a positive or a negative sentiment, we follow the heuristic introduced by \cite{rutherford2015improving}
and look for all sentences in $C$ that start with $l \in L$ followed by a comma.
We then remove $l$ and the comma from the beginning of each sentence, and annotate all resultant sentences with the class label associated with $l$. 
This process results in a binary classification dataset for sentiment analysis, which is used to fine-tune a pre-trained language model, $M$ (\textit{inter-training}).
In this work we implement the above flow using several corpora and DM lists as detailed later. 

\subsection{The \genmodel{} model} 
%The most general DM-based sentiment model, \genmodel{}, is obtained using the general corpus, \gencorpus{}, and a core list of sentiment related DMs obtained manually using general knowledge of the English language (see table \ref{tab:models}).
We first introduce \genmodel{}, a general sentiment model, that aims to improve performance of sentiment classification across domains. \genmodel{} is obtained using the flow described above, where $C$ is a general corpus of newspaper and journal articles, denoted \gencorpus{} (see section \ref{sec:corpora}), 
and $L$ is a core list of sentiment related DMs obtained manually using general knowledge of the English language. % (see table \ref{tab:models}). 
More specifically, we asked $3$ annotators, to go over a list of $173$ frequent DMs described in \cite{sileo-etal-2019-mining}, and mark any DM as positive/negative if it is likely to begin a sentence bearing a positive/negative sentiment, based on its common usage in the English language. The final list, $L_{g}$, listed in table \ref{tab:domaindms} (first row), consists of $11$ DMs, selected by all $3$ annotators. 
%More specifically, we manually select a list $L_{g}$ of discourse markers, which signal either a positive or a negative sentiment, from the Discovery list of the $173$ most frequent DMs \cite{}. The selection was performed independently by $3$ annotators asked to mark DMs that are likely to begin a sentence bearing a positive/negative sentiment, based on general English knowledge. The final list consists of $11$ DMs, selected by all $3$ annotators, listed in table \ref{tab:domaindms} -- first row (Multi domain). Each marker in $L_{g}$ is assigned to either the positive or the negative sentiment class based on its common usage in the language. For example, 'fortunately' and 'sadly' are mapped onto the positive and negative sentiment class respectively.
We fine tune both the uncased base and tiny architectures of BERT 
\cite{bert} \cite{jiao-etal-2020-tinybert}, 
%\cite{bert, jiao-etal-2020-tinybert}, 
and denote the resulting models by \genmodelbase{} and \genmodeltiny{} respectively. 
We release both of these models as part of this paper.


\begin{table}[ht!]
\begin{center}
\renewcommand{\arraystretch}{1.6}
\begin{tabular}{p{2cm}| p{0.6cm} |p{0.6cm} |p{1.3cm} | p{1.5cm}} 
 \hline
 \textbf{Model name}
 & \textbf{C} & \textbf{L} & \textbf{M} & \textbf{With self-training} \\ 
 \hline
 \genmodel & $C_g$ & $L_g$ & BERT & NA\\ 
 \hline\hline
\dmodelLg & $C_d$ & $L_g$  & \genmodel & No\\
 \hline
 \dmodelLd & $C_d$ & $L_d$ & \genmodel & No\\
 \hline
 \dmodelp & $C_d$ & NA  & \genmodel & Yes\\
 \hline
\dmodelLgP & $C_d$ & $L_g$  & \genmodel & Yes\\
 \hline
 \dmodelLdP & $C_d$ & $L_d$ & \genmodel & Yes\\
 \hline
\end{tabular}
\end{center}
%\caption{Sentiment language models and the corresponding assignment of $C$, $L$ and $M$ in the flow described in figure \ref{fig:sketch}, as well as whether the high confidence predictions of \genmodel{} are used to assign the weak labels (one step self-training), either on their own (\dmodelLg{}) or in conjunction with the predictions based on the DMs (\dmodelLgP{} and \dmodelLdP{}). \genmodel{} is a multi-domain model. The other five are domain specific. $C_g$ is a multi-domain corpus; $C_d$ is a corpus from domain $d$; $L_g$ is a list of DMs associated with sentiment in the English language; $L_d$ is such a list adapted to domain $d$.
%\ranit{consider shortening and referring to the text for details}
%\label{tab:models}
%}
\caption{Sentiment language models and the corresponding assignment of $C$, $L$ and $M$ in the flow described in figure \ref{fig:sketch}, as well as whether the predictions of \genmodel{} are used for assigning weak labels ("With self-training" -- see main text for details) . \genmodel{} is a general (multi-domain) model. The other five are domain specific. $C_g$: a general, multi-domain, corpus; $C_d$: a corpus from domain $d$; $L_g$: a list of DMs associated with sentiment in the English language; $L_d$: such a list adapted to domain $d$.
\label{tab:models}
}
\end{table}

%optional: discuss how to get an even better general model by two methods (1) expand DM list (2) use the sentiment model to label more sentences and do self training

%\subsection{Domain Specific Sentiment Models}
\subsection{Adapting \genmodel{} to a New Domain}
\label{sec:dssentmodels}
\ranit{changed a lot in this section following lena's input that the jump between model and DM (which is easly confused w model) and back to model is confusing}
In the previous section we described how $L_{g}$ can be used to train the general sentiment model, \genmodel{}. 
The generality of this model emerges from the multi-domain corpus it relies on, and the general nature of the DM list, $L_{g}$, which is composed of discourse markers that are abundantly used and have a clear sentiment association across many domains. 
However, due to potential domain-specific jargon and language style, given a domain specific text corpus $C_d$, it may be useful to build domain specific sentiment models.
%We can also expect that the sentiment-related DMs are domain specific and hence we develop a method, described in the next section, which leverages \genmodel{}, to extract from $C_d$ a domain-specific sentiment-related DM list $L_d$ that is better aligned with domain $d$.

In this work we study five ways to build domain specific sentiment models based on the flow described in figure \ref{fig:sketch}. 
All five models, described in the bottom part of table \ref{tab:models}, are based on weakly labeled sentences from the domain-specific corpus, $C_d$, and inter-training over \genmodel{} instead of BERT.
The first, \dmodelLg{}, uses the general DM list, $L_g$, for weak label extraction. 
However, we can also expect that the sentiment-related DMs are domain specific, and hence we develop a method, described in the next section, to extract a domain-specific sentiment-related DM list, $L_d$, that is better aligned with domain $d$.
The second model, \dmodelLd{}, uses this list instead $L_g$.

%Another approach is to perform one step self-training, 
Since at this stage we have a general sentiment model available, we may leverage it to further improve the weak labeling. Thus, another approach is to perform one step self-training, 
where the high confidence predictions of \genmodel{} over sentences from $C_d$ are used for inter-training, ignoring the DMs\footnote{In this work we use predictions with $score>0.9$ and $score<0.1$ as positive/negative weak labels}. This model is denoted by \dmodelp{}. 
Finally, we ask whether a synergistic approach, i.e. taking as positive/negative sentences only those for which the opening DM predicts a sentiment and that sentiment is consistent with the high confidence prediction of \genmodel{}. We thus study two additional models, \dmodelLgP{} and \dmodelLdP{}.

\subsection{Domain Specific Sentiment-Related DMs}
\label{sec:domainDMs}
We now turn to describe how we generate the domain specific sentiment-related DM list, $L_d$, given the domain specific corpus $C_d$ and using \genmodel{}. 
Importantly, we are not interested in identifying all domain specific sentiment related DMs. Rather, we are seeking a precision oriented list, for the purpose of obtaining a weakly labeled set of sentences to perform the inter-training process. Thus, we perform strict automatic filtering in the process.  
The idea is to first identify all n-grams that may potentially serve as DMs, and then identify whether the set of sentences they open is enriched with positive/negative sentiment, based on the prediction of \genmodel{}.

The first step consists of \textbf{identifying a list of candidate DMs}. To this end we first identify all unigrams, bigrams and trigrams, that, followed by a comma, open sentences in $C_d$, and further group these using NER (e.g. instead of multiple bigrams of the type "on Sept 9th", "on 10/2/2020",... we generate one bigram "on DATE"). The candidate list consists of the $1000$ most frequent DMs. Specific filters may be further applied depending on the domain corpora -- see appendix for details.

The second step consists of \textbf{using \genmodel{} to select the domain-specific DMs out of the candidate list}. 
We analyse the sentences that start with the DMs in the above candidate list, to find those DMs whose sentences are significantly associated with a positive/negative sentiment. We sample $1000$ sentences from the set of all sentences that start with the DM followed by a comma, and assign it a sentiment if it is scored with high confidence\footnote{$<0.1$ or $>0.9$} by \genmodel{}. The other sentences are considered an undecided sentiment.
For each candidate DM, we perform a statistical analysis of the sentiment of its following sentences, on the sample of $1000$ sentences, provided that they are not too repetitive based on token counts, and that the sentiment class with the higher count comprises at least $85\%$ of the sentences assigned a sentiment. 
A DM is considered to be associated with a positive/negative sentiment if the p-value of the positive/negative class is smaller than $0.01$ after Bonferroni correction for multiple tests, based on a Hypergeometric test.
%Finally, if more than $30$ sentiment DMs are identified, we keep the top $30$ DMs for each sentiment class based on p-value.
\ranit{see the comneted out sentence re 30 as a limit. none of the lists in the table reaches 30 so why do we need it. If we do need it then need to verify the last sentence is correct. also verify this entire section.}

\ranit{do we want to say we release the code for doing this? all that is needed as input is Cd and sendm right?}
\ranit{if we go for the above version we may want to add more details in the appendix. need to look carefully}

% BELOW IS THE SECTION (ALMOST) AS WE HAD IT. ABOVE IS MY ATTEMPT AT A NEW WAY TO DO IT
% \subsection{Domain Specific Sentiment-Related DMs}
% \label{sec:domainDMs}
% We now turn to describe how we generate the domain specific sentiment-related DM list, $L_d$, given the domain specific corpus $C_d$ and using \genmodel{}. 
% The idea is to first identify all n-grams that may potentially serve as DMs, and then identify whether the set of sentences they open is enriched with positive/negative sentiment, based on the prediction of \genmodel{}.
% Below we detail the process:

% \paragraph{Step 1: Generating the list of candidate domain-specific DMs.}
% We first identify all unigrams, bigrams and trigrams, that, followed by a comma, open sentences in $C_d$. 
% Since many such n-grams include named entities such as organisation names or dates, we group these n-grams using NER, e.g. instead of multiple bigrams of the type "on Sept 9th", "on 10/2/2020",... we generate one bigram "on DATE".
% Next, we measure the frequency of each candidate by counting the number of sentences that it opens, and keep the $1000$ most frequent candidates. 
% The resultant list of DM candidates is denoted by $L_d^{cand}$.
% \ranit{note next sentence and what moved to appendix}.
% Specific filters may be further applied depending on the specific domain corpora -- see appendix for details.

% \paragraph{Step 2: Using \genmodel{} to select the domain-specific DMs.}
% \ranit{consider writing this in short and moving details to exp setup. Plus can we say we will give the code that does the entire process of domain specific DMs? Maybe write it as a list of requirements that is short. Also maybe explain that the point is NOT to find all DMs associated in the domain, rather get a precision oriented list for the purpose of traning the model and hence we do severe filtering. instead of this story of 30 percent just say that we select 1000 sentences and ensure they are not repetitive based on token counts}
% We perform statistical analyses over the sentences that start with the DMs in $L_d^{cand}$ to find those DMs whose sentences are significantly associated with a positive/negative sentiment.
% For each $c \in L_d^{cand}$, we sample $1000$ sentences from the set of all sentences that starts with $c$ followed by a comma, remove it from the beginning of the sentences, and assign each sentence the Score given by \genmodel{}.
% To improve robustness to noisy predictions, for the purpose of the DM scoring, 
% we define positive and negative sentiment as only high confidence predictions, while all other sentences are considered undecided.
% %we define positive sentiment as $Score_c>=0.9$, negative as $Score_c<=0.1$, and undecided for all other values.
% Denote by $n_{pos(c)}$, $n_{neg(c)}$ and $n_{undecided(c)}$ the number of sentences corresponding to each of the above ranges respectively.
% %To find the DMs which are associated with positive/negative sentences, 
% we use the Hypergeometric test to compute a p-value indicating whether the sentences starting with $c$ are enriched with high positive/negative scores compared to the entire population. After Bonferroni correction for multiple tests, we keep only DMs with p-value smaller than $0.01$ for either the positive or the negative class, and further require that the p-value of the "undecided" class is larger than $0.2$ to avoid DMs that are enriched with non-confident predictions, which are more prone to prediction errors.
% Furthermore, we require that the sentiment class of the DM, comprises at least $85\%$ of the positive and negative sentences.
% We note that in some domains, for many DMs, the sentences they open tend to be very repetitive and hence the statistics about the p-value is not robust. We therefore ignore the $30\%$ DMs for which the number of distinct tokens (excluding non-English words and stop words based on NLTK) appearing in its $1000$ sentences divided by the total number of tokens, is lowest.
% Finally, we take up to $30$ DMs for each sentiment class.


